An Architecture for Deep, Hierarchical Generative Models

We present an architecture which lets us train deep, directed generative models with many layers of latent variables. We include deterministic paths between all latent variables and the generated output, and provide a richer set of connections between computations for inference and generation, which enables more effective communication of information throughout the model during training. To improve performance on natural images, we incorporate a lightweight autoregressive model in the reconstruction distribution. These techniques permit end-to-end training of models with 10+ layers of latent variables. Experiments show that our approach achieves state-of-the-art performance on standard image modelling benchmarks, can expose latent class structure in the absence of label information, and can provide convincing imputations of occluded regions in natural images.

==> MATNET-Extensions.tex <==
%!TEX root = MATNET-Root.tex




==> MATNET-ExtraImages.tex <==
%!TEX root = MATNET-Root.tex

\begin{figure}
\vspace{-0.25cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/face_close_1.png}}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/face_close_2.png}}
\label{fig:real_image_results}
\end{center}
\vspace{-0.25cm}
\end{figure}

\begin{figure}
\vspace{-0.25cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/face_close_3.png}}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/face_close_4.png}}
\label{fig:real_image_results}
\end{center}
\vspace{-0.25cm}
\end{figure}

\begin{figure}
\vspace{-0.25cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/church_close_1.png}}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/church_close_2.png}}
\label{fig:real_image_results}
\end{center}
\vspace{-0.25cm}
\end{figure}

\begin{figure}
\vspace{-0.25cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/church_close_3.png}}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/church_close_4.png}}
\label{fig:real_image_results}
\end{center}
\vspace{-0.25cm}
\end{figure}

\begin{figure}
\vspace{-0.25cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/tower_close_1.png}}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/tower_close_2.png}}
\label{fig:real_image_results}
\end{center}
\vspace{-0.25cm}
\end{figure}

\begin{figure}
\vspace{-0.25cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/tower_close_3.png}}
  \subfigure[]{\includegraphics[scale=0.62]{./figures/tower_close_4.png}}
\label{fig:real_image_results}
\end{center}
\vspace{-0.25cm}
\end{figure}

==> MATNET-RelatedWork.tex <==
%!TEX root = MATNET-Root.tex

Matryoshka Networks concretely instantiate an idea we call \emph{deconstruction/reconstruction processes}. Dec/rec processes provide a natural approach to constructing deep, hierarchical directed generative models with many layers of latent variables. 

Hierarchically deep models have also been trained using a class of methods which we call \emph{deconstruction/reconstruction processes}. Intuitively, one can think of the primary mechanism behind dec/rec processes as akin to solving mazes by starting at the end and working backwards, or to learning how an object works by repeatedly disassembling and reassembling it. This encompasses methods such as the LapGANs introduced by \cite{Denton2015}, which deconstruct an image by repeatedly downsampling it, and the Diffusion Nets introduced by \cite{SohlDickstein2015}, which deconstruct arbitrary data by subjecting it to random perturbations.

Discuss relations between dec/rec processes and the interpretations and motivations of inference promulgated by Tenebaum's cohort. Mention \citet{Lake2015} and \citet{Eslami2016}.


The power of dec/rec processes stems from the way in which the deconstruction process leaves behind a trail of bread crumbs, which can be followed back to the original data. In the generative models of \cite{Denton2015, SohlDickstein2015}, the deconstruction processes were defined a priori, which avoided the need for trained inference. Defining the deconstruction (i.e.~inference) process a priori makes training significantly easier by eliminating the need for synchronization between inference and generation, thereby allowing the generator to focus on (stochastically) inverting the deconstruction process. Though practically convenient, this approach subverts one of the main motivations for working with latent variables and sample-based approximate inference --- the ability to capture salient factors of variation in the inferred relations between latent variables and observed data.

Write about related work. Don't rock the boat, all aboard the hype train -- choo choo.

Among recently developed approaches to training generative models, we consider the most promising to be: stochastic variational methods for directed generative models \citep{Kingma2014a, Rezende2014}, adversarial techniques which provide an alternative to maximum-likelihood/maximum-a-posteriori methods \citep{Goodfellow2014, Denton2015, Radford2016}, and methods which build on the autoregressive approach introduced by \cite{Larochelle2011}, e.g.~\citep{Gemain2015, VanDenOord2016}.




==> MATNET-Tables.tex <==
%!TEX root = MATNET-Root.tex

\clearpage
\clearpage
\clearpage
\clearpage

\begin{table}[t]
	\small
	\centering
    \begin{tabular}{| l || c | c | c |}
    	\hline
    	Method & 1 quadrant & 2 quadrants & 3 quadrants \\
    	 \hline
    	 NN & 99.75 & 62.18 & 25.99 \\
    	 GSNN & 99.82 & 62.41 & 26.29 \\
    	 CVAE & 68.39 & 45.34 & 20.96 \\
    	 CVAE & 63.91 & 44.73 & 20.95 \\ 
    	 MatNet & 57.45 & 36.82 & 17.96 \\ \hline
	 \multicolumn{4}{l}{Structured prediction NLL with $n$ quadrants visible \cite{Sohn2015}} \\
    \end{tabular}
	\label{tab:cll}
\end{table}

\begin{table}[t]
	\small
	\centering
    \begin{tabular}{  l c }
    	\hline
		\textbf{Model} & \textbf{Test NLL} \\ \hline

		VAE (2 layers, 5 samples) & 106.31 \\
		
		IWAE (2 layers, 50 samples) & 103.38 \\
		
		RBM (500 hidden) & 100.46 \\ \hline
		
		DRAW & $< 96.5$ \\
		
		Conv DRAW & $< 91.0$ \\ \hline
		
		MatNet & $< 89.5$ \\	
		\hline
    \end{tabular}
    \caption{NLL on 28x28 Omniglot.}
	\label{tab:omni_nll}
\end{table}

\begin{table}[t]
	\small
	\centering
    \begin{tabular}{  l c }
    	\hline
		\textbf{Model} & \textbf{Test NLL} \\ \hline
		Uniform Distribution & 8.00 \\
		Multivariate Gaussian & 4.70 \\
		NICE~\citep{Dinh2015} & 4.48 \\
		Deep Diffusion~\citep{SohlDickstein2015} & 4.20 \\
		Deep GMMs~\citep{VanDenOord2014} & 4.00 \\
		Pixel RNN~\citep{VanDenOord2016} & 3.00 \\ \hline
		DRAW & $< 4.13$ \\
		Conv DRAW & $< 3.58$ \\ \hline
		MatNet & $< 3.68$ \\
		MatNet+AR & $< 3.24$ \\
		\hline
    \end{tabular}
    \caption{NLL on CIFAR 10.}
	\label{tab:cifar10_nll}
\end{table}

\begin{table}[t]
	\small
	\centering
    \begin{tabular}{ c c c }
    	\hline
    	\multicolumn{2}{c}{\textbf{Model}} & \textbf{Test NLL} \\  \hline
    	\multicolumn{2}{l}{DRAW (64 steps, Gaussian attention)} & $\leq 80.9$ \\
	    \multicolumn{2}{l}{DRAW (80 steps, ST att and CGRU canvas)} & $\leq 80.5$ \\
	    \multicolumn{2}{l}{Pixel RNN} & $\leq 79.2$ \\ \hline
	    \multicolumn{2}{l}{MatNet} & $\leq 78.5$
    \end{tabular}
    \caption{NLL on MNIST -- Convolutional.}
	\label{tab:mnist_nll}
\end{table}

\begin{table}[t]
	\small
	\centering
    \begin{tabular}{ c c c }
    	\hline
    	\multicolumn{2}{c}{\textbf{Model}} & \textbf{Test NLL} \\  \hline
    	\multicolumn{2}{l}{DRAW (16 steps, no attention) \cite{Gregor2015}} & $\leq 87.4$ \\
	    \multicolumn{2}{l}{VAE + IWAE \cite{Burda2015}} & $\leq 82.9$ \\
	    \multicolumn{2}{l}{Prob Ladder \cite{Sonderby2016}} & $\leq 81.2$ \\ \hline
	    \multicolumn{2}{l}{FC MatNet} & $\leq 80.5$
    \end{tabular}
    \caption{NLL on MNIST -- Fully-connected.}
	\label{tab:mnist_nll}
\end{table}
